Adversarial Regression with Multiple Learners

Despite the considerable success enjoyed by machine learning techniques in practice, numerous studies demonstrated that many approaches are vulnerable to attacks. An important class of such attacks involves adversaries changing features at test time to cause incorrect predictions. Previous investigations of this problem pit a single learner against an adversary. However, in many situations an adversary's decision is aimed at a collection of learners, rather than specifically targeted at each independently. We study the problem of adversarial linear regression with multiple learners. We approximate the resulting game by exhibiting an upper bound on learner loss functions, and show that the resulting game has a unique symmetric equilibrium. We present an algorithm for computing this equilibrium, and show through extensive experiments that equilibrium models are significantly more robust than conventional regularized linear regression.

==> section/robustness__Yevgeniy_Vorobeychik_s_conflicted_copy_2018-02-08_.tex <==
\section{Robustness Analysis}
\label{sec:robust}



We then analyze the robustness of the learners using the techniques introduced in \cite{xu2009robust}. Specifically, we prove the equivalence between Eq.~\eqref{eq:solution} and a robust linear regression problem where data  is maliciously corrupted by some disturbance $\boldsymbol{\triangle}$, which results in a min-max problem as Eq.\eqref{eq:min_max}. From a game-theoretic point of view, in training phase the defender is simulating an attacker. The attacker maximizes the training error by adding disturbance to $\mathbf{X}$. The magnitude of the disturbance is controlled by a parameter $c=\frac{\beta(n+1)}{2\lambda^2}{|| \mathbf{z}- \mathbf{y} ||_2^2}$. Remember  $\lambda$, $\beta$ and $\mathbf{z}$ are externally set by the attacker. So  Eq.\eqref{eq:min_max}  the fundamental reason that \textit{MLSG} is robust is because it proactively takes adversarial behavor into account in training phrase. 


\begin{theorem}
\label{thm:robustness}
The optimization problem presented in Eq.~\eqref{eq:solution} is equivalent to the followring robust optimization problem with the uncertainty set $\mathcal{U}=\{ \boldsymbol{\triangle} \in \mathbb{R}^{m \times d} \, | \, {\boldsymbol{\triangle}}^T{\boldsymbol{\triangle}}=\mathbf{G}: \forall i\ne j, \,\, \mathbf{G}_{ii} \le c {|\bm{\theta}^{\ast}_i|}^2  \text{ and } sign(\tau)\mathbf{G}_{ij} \le  sign(\tau)\tau c \}$, where $c=\frac{\beta(n+1)}{2\lambda^2}{|| \mathbf{z}- \mathbf{y} ||_2^2}$, $\tau=\bm{\theta}^{\ast}_i \bm{\theta}^{\ast}_j$, $sign(\cdot)$ is the sign function and $\bm{\theta}^{\ast}$ is the optimal solution of Eq.~\eqref{eq:solution}.
	\begin{equation}\label{eq:min_max}
		\min_{\bm{\theta} \in \bm{\Theta}} \max_{\boldsymbol{\triangle} \in \mathcal{U}} {|| \mathbf{y} - (\mathbf{X} + \boldsymbol{\triangle})\bm{\theta}   ||_2^2}
	\end{equation}
\end{theorem}
\begin{proof}
Fix $\bm{\theta}^{\ast}$, we show that $\max_{\boldsymbol{\triangle} \in \mathcal{U}} {|| \mathbf{y} - (\mathbf{X} + \boldsymbol{\triangle})\bm{\theta}^{\ast}   ||}_2^2 = {|| \mathbf{y} - \mathbf{X}\bm{\theta}^{\ast} ||_2^2} + c{( {\bm{\theta}^{\ast}}^T \bm{\theta}^{\ast}   )}^2$. The left-hand side can be expanded as: 
		\begin{align}
			\begin{split}
				& \max_{\boldsymbol{\triangle} \in \mathcal{U}} {|| \mathbf{y} - (\mathbf{X} + \boldsymbol{\triangle})\bm{\theta}^{\ast}   ||_2^2} \\
			 =  & \max_{\boldsymbol{\triangle} \in \mathcal{U}} {||  \mathbf{y} - \mathbf{X}\bm{\theta}^{\ast} - \boldsymbol{\triangle}\bm{\theta}^{\ast} ||_2^2} \\
			 \le &  \max_{\boldsymbol{\triangle} \in \mathcal{U}} {||\mathbf{y} - \mathbf{X}\bm{\theta}^{\ast} ||_2^2} +  \max_{\boldsymbol{\triangle} \in \mathcal{U}} { || \boldsymbol{\triangle} \bm{\theta}^{\ast} ||_2^2 } \\ 
			 = & \max_{\boldsymbol{\triangle} \in \mathcal{U}} {||\mathbf{y} - \mathbf{X}\bm{\theta}^{\ast} ||_2^2} + \max_{\boldsymbol{\triangle} \in \mathcal{U}} { {\bm{\theta}^{\ast}}^T {\boldsymbol{\triangle}}^T{\boldsymbol{\triangle}}  \bm{\theta}^{\ast}} \\
			 & \text{substitute ${\boldsymbol{\triangle}}^T{\boldsymbol{\triangle}}=\mathbf{G}$} \\
			 = &  {||\mathbf{y} - \mathbf{X}\bm{\theta}^{\ast} ||_2^2} + \max_{\mathbf{G} } {{\bm{\theta}^{\ast}}^T \mathbf{G} \bm{\theta}^{\ast}} \\
			 = &  {||\mathbf{y} - \mathbf{X}\bm{\theta}^{\ast} ||_2^2}  +  \max_{\mathbf{G} } {\sum_{i=1}^{d}{ {|\bm{\theta}^{\ast}_i|}^2 \mathbf{G}_{ii}  }  } + {2\sum_{j=1}^{d}{   \sum_{i=1}^{j-1}{  \bm{\theta}^{\ast}_i \bm{\theta}^{\ast}_j \mathbf{G}_{ij}        }        }} \\
			 \le & {||\mathbf{y} - \mathbf{X}\bm{\theta}^{\ast} ||_2^2} +  c{\sum_{i=1}^{d}{ {|\bm{\theta}^{\ast}_i|}^4  }  } + {2c\sum_{j=1}^{d}{   \sum_{i=1}^{j-1}{  (\bm{\theta}^{\ast}_i \bm{\theta}^{\ast}_j)^2      }        }} \\
			 = & {||\mathbf{y} - \mathbf{X}\bm{\theta}^{\ast} ||_2^2} + c\big( \sum_{i=1}^{d}{|\bm{\theta}^{\ast}_i|^2} \big)^2 \\
			 = & {||\mathbf{y} - \mathbf{X}\bm{\theta}^{\ast} ||_2^2} + c{( {\bm{\theta}^{\ast}}^T \bm{\theta}^{\ast}   )}^2
			\end{split}
		\end{align}


Now we define $\boldsymbol{\triangle}^{\ast}=[\sqrt{c}\bm{\theta}^{\ast}_1 \mathbf{u},\cdots,\sqrt{c}\bm{\theta}^{\ast}_n \mathbf{u}]$, where $\bm{\theta}^{\ast}_i$ is the $i$-th element of $\bm{\theta}^{\ast}$ and $\mathbf{u}$ is:
  \begin{equation}
    \mathbf{u} \triangleq
    \begin{cases}
	       \frac{\mathbf{y} - \mathbf{X}\bm{\theta}^{\ast}}{|| \mathbf{y} - \mathbf{X}\bm{\theta}^{\ast} ||_2}, &  \textit{if}\ \mathbf{y} \ne \mathbf{X}\bm{\theta}^{\ast} \\
	      \textit{any vector with unit $L_2$ norm}, & \text{otherwise}
	    \end{cases}
  \end{equation}

Then we have:
		\begin{align}
			\begin{split}
			    & \max_{\boldsymbol{\triangle} \in \mathcal{U}} {|| \mathbf{y} - (\mathbf{X} + \boldsymbol{\triangle})\bm{\theta}^{\ast}   ||}_2^2 \\
			\ge &  {|| \mathbf{y} - (\mathbf{X} + \boldsymbol{\triangle}^{\ast})\bm{\theta}^{\ast}   ||}_2^2 \\
			=   & {|| \mathbf{y} - \mathbf{X}\bm{\theta}^{\ast} - \boldsymbol{\triangle}^{\ast}\bm{\theta}^{\ast}   ||}_2^2 \\
			= & {|| \mathbf{y} - \mathbf{X}\bm{\theta}^{\ast} - \sum_{i=1}^{d}{  \sqrt{c}|\bm{\theta}^{\ast}_i|^2 \mathbf{u}    }  ||_2^2} \\
			& \text{($\mathbf{u}$ is in the same direction as $\mathbf{y} - \mathbf{X}\bm{\theta}^{\ast}$ )} \\
			= & {|| \mathbf{y} - \mathbf{X}\bm{\theta}^{\ast} ||_2^2} + {||  \sum_{i=1}^{d}{  \sqrt{c}|\bm{\theta}^{\ast}_i|^2 \mathbf{u}    }  ||_2^2} \\
			= & {|| \mathbf{y} - \mathbf{X}\bm{\theta}^{\ast} ||_2^2} + c{( {\bm{\theta}^{\ast}}^T \bm{\theta}^{\ast}   )}^2
			\end{split}
		\end{align}
\end{proof} 

% \bm{\theta}^{\ast}

==> section/robustness__Yevgeniy_Vorobeychik_s_conflicted_copy_2018-02-08__1__.tex <==
\section{Robustness Analysis}
\label{sec:robust}

We now draw a connection between the multi-learner equilibrium in the adversarial setting, derived above, and robustness, in the spirit of the analysis by \citet{xu2009robust}.
%We then analyze the robustness of the learners using the techniques introduced in \cite{xu2009robust}. 
Specifically, we prove the equivalence between Eq.~\eqref{eq:solution} and a robust linear regression problem where data is maliciously corrupted by some disturbance $\boldsymbol{\triangle}$.
Formally, a robust linear regression solves the following problem:
	\begin{equation}\label{eq:min_max}
		\min_{\bm{\theta} \in \bm{\Theta}} \max_{\boldsymbol{\triangle} \in \mathcal{U}} {|| \mathbf{y} - (\mathbf{X} + \boldsymbol{\triangle})\bm{\theta}   ||_2^2},
	\end{equation}
where the uncertainty set $\mathcal{U}=\{ \boldsymbol{\triangle} \in \mathbb{R}^{m \times d} \, | \, {\boldsymbol{\triangle}}^T{\boldsymbol{\triangle}}=\mathbf{G}: \forall i\ne j, \,\, \mathbf{G}_{ii} \le c {|\bm{\theta}^{\ast}_i|}^2  \text{ and } sign(\tau)\mathbf{G}_{ij} \le  sign(\tau)\tau c \}$, with $c=\frac{\beta(n+1)}{2\lambda^2}{|| \mathbf{z}- \mathbf{y} ||_2^2}$, $\tau=\bm{\theta}^{\ast}_i \bm{\theta}^{\ast}_j$, $sign(\cdot)$ is the sign function, and with $\bm{\theta}^{\ast}$ the optimal solution of Eq.~\eqref{eq:solution}.

%which results in a min-max problem shown in Eq.\eqref{eq:min_max}. 
From a game-theoretic point of view, in training phase the defender is simulating an attacker. The attacker maximizes the training error by adding disturbance to $\mathbf{X}$. The magnitude of the disturbance is controlled by a parameter $c=\frac{\beta(n+1)}{2\lambda^2}{|| \mathbf{z}- \mathbf{y} ||_2^2}$. Consequently, the robustness of Eq.~\eqref{eq:min_max} is guaranteed if and only if the magnitude reflects the uncertainty interval. This sheds some light on how to choose $\lambda$, $\beta$ and $\mathbf{z}$ in practice. One strategy is to over-estimate the attacker's strength, which amounts to choosing small values of $\lambda$, large values of $\beta$ and exaggerated target $\mathbf{z}$. The intuition of this strategy is to enlarge the uncertainty set so as to cover potential adversarial behavior. In the experiments we will show that this strategy works well in practice. 
Eq.~\eqref{eq:min_max} also offers us an insight about the fundamental reason \textit{MLSG} is robust (as we observe in the experiments).


% Remember  $\lambda$, $\beta$ and $\mathbf{z}$ are externally set by the attacker. So  Eq.\eqref{eq:min_max}  the fundamental reason that \textit{MLSG} is robust is because it proactively takes adversarial behavor into account in training phrase. 

\begin{theorem}
\label{thm:robustness}
The optimal solution $\bm{\theta}^{\ast}$ of the problem in Eq.~\eqref{eq:solution} is an optimal solution to the robust optimization problem in Eq.~\eqref{eq:min_max}.
%the followring robust optimization problem with the uncertainty set $\mathcal{U}=\{ \boldsymbol{\triangle} \in \mathbb{R}^{m \times d} \, | \, {\boldsymbol{\triangle}}^T{\boldsymbol{\triangle}}=\mathbf{G}: \forall i\ne j, \,\, \mathbf{G}_{ii} \le c {|\bm{\theta}^{\ast}_i|}^2  \text{ and } sign(\tau)\mathbf{G}_{ij} \le  sign(\tau)\tau c \}$, where $c=\frac{\beta(n+1)}{2\lambda^2}{|| \mathbf{z}- \mathbf{y} ||_2^2}$, $\tau=\bm{\theta}^{\ast}_i \bm{\theta}^{\ast}_j$, $sign(\cdot)$ is the sign function and $\bm{\theta}^{\ast}$ is the optimal solution of Eq.~\eqref{eq:solution}.
\end{theorem}

\begin{proof}
Fix $\bm{\theta}^{\ast}$, we show that $\max_{\boldsymbol{\triangle} \in \mathcal{U}} {|| \mathbf{y} - (\mathbf{X} + \boldsymbol{\triangle})\bm{\theta}^{\ast}   ||}_2^2 = {|| \mathbf{y} - \mathbf{X}\bm{\theta}^{\ast} ||_2^2} + c{( {\bm{\theta}^{\ast}}^T \bm{\theta}^{\ast}   )}^2$. The left-hand side can be expanded as: 
		\begin{align*}
%			\begin{split}
				& \max_{\boldsymbol{\triangle} \in \mathcal{U}} {|| \mathbf{y} - (\mathbf{X} + \boldsymbol{\triangle})\bm{\theta}^{\ast}   ||_2^2} \\
			 =  & \max_{\boldsymbol{\triangle} \in \mathcal{U}} {||  \mathbf{y} - \mathbf{X}\bm{\theta}^{\ast} - \boldsymbol{\triangle}\bm{\theta}^{\ast} ||_2^2} \\
			 \le &  \max_{\boldsymbol{\triangle} \in \mathcal{U}} {||\mathbf{y} - \mathbf{X}\bm{\theta}^{\ast} ||_2^2} +  \max_{\boldsymbol{\triangle} \in \mathcal{U}} { || \boldsymbol{\triangle} \bm{\theta}^{\ast} ||_2^2 } \\ 
			 = & \max_{\boldsymbol{\triangle} \in \mathcal{U}} {||\mathbf{y} - \mathbf{X}\bm{\theta}^{\ast} ||_2^2} + \max_{\boldsymbol{\triangle} \in \mathcal{U}} { {\bm{\theta}^{\ast}}^T {\boldsymbol{\triangle}}^T{\boldsymbol{\triangle}}  \bm{\theta}^{\ast}} \\
			 & \text{substitute ${\boldsymbol{\triangle}}^T{\boldsymbol{\triangle}}=\mathbf{G}$} \\
			 = &  {||\mathbf{y} - \mathbf{X}\bm{\theta}^{\ast} ||_2^2} + \max_{\mathbf{G} } {{\bm{\theta}^{\ast}}^T \mathbf{G} \bm{\theta}^{\ast}} \\
			 = &  {||\mathbf{y} - \mathbf{X}\bm{\theta}^{\ast} ||_2^2}  +  \max_{\mathbf{G} } {\sum_{i=1}^{d}{ {|\bm{\theta}^{\ast}_i|}^2 \mathbf{G}_{ii}  }  } + {2\sum_{j=1}^{d}{   \sum_{i=1}^{j-1}{  \bm{\theta}^{\ast}_i \bm{\theta}^{\ast}_j \mathbf{G}_{ij}        }        }} \\
			 \le & {||\mathbf{y} - \mathbf{X}\bm{\theta}^{\ast} ||_2^2} +  c{\sum_{i=1}^{d}{ {|\bm{\theta}^{\ast}_i|}^4  }  } + {2c\sum_{j=1}^{d}{   \sum_{i=1}^{j-1}{  (\bm{\theta}^{\ast}_i \bm{\theta}^{\ast}_j)^2      }        }} \\
			 = & {||\mathbf{y} - \mathbf{X}\bm{\theta}^{\ast} ||_2^2} + c\big( \sum_{i=1}^{d}{|\bm{\theta}^{\ast}_i|^2} \big)^2 \\
			 = & {||\mathbf{y} - \mathbf{X}\bm{\theta}^{\ast} ||_2^2} + c{( {\bm{\theta}^{\ast}}^T \bm{\theta}^{\ast}   )}^2.
%			\end{split}
		\end{align*}

Define $\boldsymbol{\triangle}^{\ast}=[\sqrt{c}\bm{\theta}^{\ast}_1 \mathbf{u},\cdots,\sqrt{c}\bm{\theta}^{\ast}_n \mathbf{u}]$, where $\bm{\theta}^{\ast}_i$ is the $i$-th element of $\bm{\theta}^{\ast}$ and $\mathbf{u}$ is:
  \begin{equation}
    \mathbf{u} \triangleq
    \begin{cases}
	       \frac{\mathbf{y} - \mathbf{X}\bm{\theta}^{\ast}}{|| \mathbf{y} - \mathbf{X}\bm{\theta}^{\ast} ||_2}, &  \textit{if}\ \mathbf{y} \ne \mathbf{X}\bm{\theta}^{\ast} \\
	      \textit{any vector with unit $L_2$ norm}, & \text{otherwise}
	    \end{cases}
  \end{equation}
Then we have:
		\begin{align}
			\begin{split}
			    & \max_{\boldsymbol{\triangle} \in \mathcal{U}} {|| \mathbf{y} - (\mathbf{X} + \boldsymbol{\triangle})\bm{\theta}^{\ast}   ||}_2^2 \\
			\ge &  {|| \mathbf{y} - (\mathbf{X} + \boldsymbol{\triangle}^{\ast})\bm{\theta}^{\ast}   ||}_2^2 \\
			=   & {|| \mathbf{y} - \mathbf{X}\bm{\theta}^{\ast} - \boldsymbol{\triangle}^{\ast}\bm{\theta}^{\ast}   ||}_2^2 \\
			= & {|| \mathbf{y} - \mathbf{X}\bm{\theta}^{\ast} - \sum_{i=1}^{d}{  \sqrt{c}|\bm{\theta}^{\ast}_i|^2 \mathbf{u}    }  ||_2^2} \\
			& \text{($\mathbf{u}$ is in the same direction as $\mathbf{y} - \mathbf{X}\bm{\theta}^{\ast}$ )} \\
			= & {|| \mathbf{y} - \mathbf{X}\bm{\theta}^{\ast} ||_2^2} + {||  \sum_{i=1}^{d}{  \sqrt{c}|\bm{\theta}^{\ast}_i|^2 \mathbf{u}    }  ||_2^2} \\
			= & {|| \mathbf{y} - \mathbf{X}\bm{\theta}^{\ast} ||_2^2} + c{( {\bm{\theta}^{\ast}}^T \bm{\theta}^{\ast}   )}^2
			\end{split}
		\end{align}
\end{proof} 

% \bm{\theta}^{\ast}
